Inference of Resource Management Specifications

A resource leak occurs when a program fails to free some finite resource after it is no longer needed. Such leaks are a significant cause of real-world crashes and performance problems. Recent work proposed an approach to prevent resource leaks based on checking resource management specifications. A resource management specification expresses how the program allocates resources, passes them around, and releases them; it also tracks the ownership relationship between objects and resources, and aliasing relationships between objects. While this specify-and-verify approach has several advantages compared to prior techniques, the need to manually write annotations presents a significant barrier to its practical adoption. This paper presents a novel technique to automatically infer a resource management specification for a program, broadening the applicability of specify-and-check verification for resource leaks. Inference in this domain is challenging because resource management specifications differ significantly in nature from the types that most inference techniques target. Further, for practical effectiveness, we desire a technique that can infer the resource management specification intended by the developer, even in cases when the code does not fully adhere to that specification. We address these challenges through a set of inference rules carefully designed to capture real-world coding patterns, yielding an effective fixed-point-based inference algorithm. We have implemented our inference algorithm in two different systems, targeting programs written in Java and C#. In an experimental evaluation, our technique inferred 85.5% of the annotations that programmers had written manually for the benchmarks. Further, the verifier issued nearly the same rate of false alarms with the manually-written and automatically-inferred annotations.

==> Makefile <==
# Put user-specific changes in your own Makefile.user.
# Make will silently continue if that file does not exist.
-include Makefile.user

# Mac OS X users may need to add to Makefile.user:
#  LATEXMK = /usr/texbin/latexmk
LATEXMK ?= latexmk

NAME	:= result

all: ${NAME}.pdf

.PRECIOUS: %.pdf
${NAME}.pdf: plume-bib-update
	latexmk -bibtex -pdf -shell-escape -synctex=1 -interaction=nonstopmode -f "${NAME}.tex"
  # Fail the build if there are undefined references or citations.
	@ ! grep "Warning: There were undefined references." "${NAME}.log"
	@ ! grep "Warning: There were undefined citations." "${NAME}.log"

${NAME}-notodos.pdf: ${NAME}.pdf
	pdflatex -shell-escape "\def\notodocomments{}\input{${NAME}}"
	pdflatex -shell-escape "\def\notodocomments{}\input{${NAME}}"
	cp -pf ${NAME}.pdf $@

# You will upload onefile.zip to the publisher website after acceptance.
onefile.zip: onefile.tex
	zip onefile.zip onefile.tex acmart.cls ACM-Reference-Format.bst
# The latex-process-inputs program is part of https://github.com/plume-lib/plume-scripts,
# which is a collection of useful scripts. I recommend adding it to your PATH.
onefile.tex:
	latex-process-inputs ${NAME}.tex > onefile.tex

# This target creates:
#   https://homes.cs.washington.edu/~mernst/tmp33333/resource-leak-inference.pdf
web: ${NAME}-notodos.pdf
	cp -pf $^ ${HOME}/public_html/tmp33333/resource-leak-inference.pdf

view: ${NAME}.pdf
	open $<

ispell: spell
spell:
	for file in `latex-process-inputs -list ${NAME}.tex`; do ispell $$file; done

# Count words in the abstract, which some conferences limit.
abs-words:
	grep -v 'Abstract' abstract.tex | egrep -v '^%' | wc -w

plume-bib:
ifdef PLUMEBIB
	ln -s ${PLUMEBIB} $@
else
	git clone https://github.com/mernst/plume-bib.git
endif
.PHONY: plume-bib-update
# Even if the plume-bib-update target fails, it does not terminate the make job.
# However, to skip it, invoke make as:  make NOGIT=1 ...
plume-bib-update: plume-bib
ifndef NOGIT
	-(cd plume-bib && git pull && make)
endif

.PHONY: tags
TAGS: tags
tags:
	etags `latex-process-inputs -list ${NAME}.tex`

clean:
	latexmk -C "${NAME}.tex"


==> plume-bib/README <==
plume-bib:  collection of BibTeX bibliography files
===================================================

To obtain the bibliographies, run:

    git clone https://github.com/mernst/plume-bib.git

This is a set of BibTeX bibliographies.  You can re-use them rather than
having to re-type or download.  Re-typing or downloading bibliography
entries is a notorious source of errors.  For example, even the ACM Digital
Library often has incorrect capitalization, or gives a SIGPLAN Notices
reference when the conference proceedings would be more appropriate.

Here are some other features:

 * Short and long versions of names, locations, and dates for conferences,
   journals, etc.  The short (abbreviated) version is convenient if your
   paper is nearing its page limit.  Changing between the two versions only
   requires a tiny change to your LaTeX file (see below), and no
   changes to any bib files.
 * Consistent naming convention for citation keys:  last name of first
   author, followed by last initial of each other author, followed by
   year.  This makes the citation more recognizable in your LaTeX source,
   and avoids duplicates.
 * Searchable via the bibfind tool.  For instance, `bibfind keyword1 keyword2`
   displays all the bibliographies with all the keywords, either in the
   entries in the comments.  (This is why there are no blank lines in the
   comments that abut some bib entries:  the search tool considers each
   blank line to start a new entry.  We may lift that restriction in the
   future.)

You can obtain the bibliographies by running the command
`git clone https://github.com/mernst/plume-bib.git`
but you don't need to -- see below for how to set your build system to
automatically obtain and/or update a copy.

You can also set the `PLUMEBIB` environment variable to the location of your
clone (usually a directory named bib), so that you will have just one clone
rather than one for each paper you write.


USAGE
-----

To choose the abbreviated (short) or unabbreviated (long) version of the
bibliography strings, use one of these commands in your LaTeX file:

    % Use either "-abbrev" or "-unabbrev" to control citation verbosity.
    \bibliography{plume-bib/bibstring-abbrev,...,plume-bib/crossrefs-abbrev}
    \bibliography{plume-bib/bibstring-unabbrev,...,plume-bib/crossrefs}

When using the bibliographies, add near the top of your LaTeX document:

    \usepackage{url}

This defines the `\url` command used in the bibliographies.  To make URLs use
a slightly narrower font (the regular `tt` font is very wide), use:

    \usepackage{pslatex}

or, to use a smaller font, use:

    \usepackage{relsize}
    \def\UrlFont{\smaller\ttfamily}


EDITING AND ADDING ENTRIES
--------------------------

Changes, corrections, and additions are welcome.

When adding new bibliography entries, please create an entry in
`crossrefs.bib` for conferences, and create bibliography strings in
`bibstring-master` for journal/institution names and abbreviations.

For consistency, please start each new bibliography entry with "@" in the
first column, and end the entry with "}" on its own line.

If you make changes but you lack write access to the Git repository at
https://github.com/mernst/plume-bib, then please submit a pull request, or
email a patch (a diff file) with your changes to Michael Ernst
<mernst@cs.washington.edu>.  Thanks for your contributions!


SETUP -- if you use a Makefile to process your paper
----------------------------------------------------

1. Add "plume-bib" as a dependency for the rule that calls bibtex; for example,
   make "plume-bib" a dependency for the myfile.bbl target.  If no rule calls
   bibtex, you can skip this step.
2. Add "plume-bib-update" as a dependency of your default target (such as "all").
3. Add the following rules to your Makefile.
   (Warning: these commands get mangled when viewing the README at GitHub.
   Clone the repository and view the `README` file directly.)

    plume-bib:
    ifdef PLUMEBIB
	    ln -s ${PLUMEBIB} $@
    else
	    git clone https://github.com/mernst/plume-bib.git $@
    endif
    .PHONY: plume-bib-update
    # Even if the plume-bib-update target fails, it does not terminate the make job.
    # However, to skip it, invoke make as:  make NOGIT=1 ...
    plume-bib-update: plume-bib
    ifndef NOGIT
	    -(cd plume-bib && git pull && make)
    endif


SETUP -- non-Makefile version
-----------------------------

If you have previously cloned plume-bib and set the PLUMEBIB environment
variable, there is nothing to do.  Otherwise, run this command:

    cd; git clone https://github.com/mernst/plume-bib.git plume-bib

Then, set the PLUMEBIB environment variable to $HOME/plume-bib and
add the "plume-bib" directory to your BIBINPUTS environment variable.

bash syntax:

    export PLUMEBIB=$HOME/plume-bib
    export BIBINPUTS=.:${PLUMEBIB}:..:


SETUP -- miscellaneous details
------------------------------

For the bibfind command, see
https://github.com/mernst/uwisdom/blob/wiki/README.adoc .
The bibfind command uses the `bibroot` file in the `plume-bib` directory.

If you wish to have only a single copy of the bibliographies on your
computer, you can clone the repository just once and set the PLUMEBIB
environment variable.  Then your Makefile will create (or you can make by
hand) a symbolic link from any directories where you are writing a paper.

Note for miktex users:
The bibtex that is supplied with miktex (the popular Windows implementation)
does not support the BIBINPUTS variable. You need to modify the miktex
configuration.  In file `...\miktex\config\miktex.ini`, edit this entry:

    Input Dirs=searchpath
    (search path for BibTeX input files -- both databases and style files).


INVOKING BIBTEX: crossref and -min-crossrefs=9999
-------------------------------------------------

plume-bib's .bib files use `@crossref`.  To avoid outut like

    [1] Brun et al.  Paper title.  In [2].
    [2] Proceedings of ESEC/FSE 2011.  Szeged, Hungary, Sep. 7--9, 2011.

you need to pass the -min-crossrefs=9999 command-line option to BibTeX; for
example:

    bibtex -min-crossrefs=9999 mypaper


LICENSE
-------

Uses the Creative Commons Attribution ("CC-BY") license.  See file LICENSE.


==> plume-bib/bibroot <==
% File for finding bibliography items.

\include{algorithms.bib}
\include{alias.bib}
\include{common-subexpr.bib}
\include{compiler.bib}
\include{concurrency.bib}
\include{continuoustesting.bib}
\include{cryptography.bib}
\include{debug-optimized.bib}
\include{dispatch.bib}
\include{education.bib}
\include{ernst.bib}
\include{ernst-underreview.bib}
\include{games.bib}
\include{garbage-collection.bib}
\include{generals.bib}
\include{heaps.bib}
\include{invariants.bib}
\include{ioa.bib}
\include{konane.bib}
\include{kvasir.bib}
\include{layout.bib}
\include{lectures-ernst.bib}
\include{macros.bib}
\include{model-checking.bib}
\include{nlp.bib}
\include{noncs.bib}
\include{other.bib}
\include{pag.bib}
\include{parallel.bib}
\include{partoseq.bib}
\include{philosophy.bib}
\include{prefetch.bib}
\include{proglang-seminar.bib}
\include{program-analysis.bib}
\include{rayside-polymorphism.bib}
\include{security.bib}
\include{semantics.bib}
\include{sideeff.bib}
\include{slicing.bib}
\include{soft-eng.bib}
\include{systems.bib}
\include{tao-of-phd.bib}
\include{testing.bib}
\include{types.bib}
\include{upgrades-ajmani.bib}
\include{upgrades-mde.bib}
\include{version-control.bib}

